Constructive characterisations of the must-preorder for asynchrony

De Nicola and Hennessy's must-preorder is a contextual refinement which states that a server q refines a server p if all clients satisfied by p are also satisfied by q. Owing to the universal quantification over clients, this definition does not yield a practical proof method for the must-preorder, and alternative characterisations are necessary to reason over it. Finding these characterisations for asynchronous semantics, i.e. where outputs are non-blocking, has thus far proven to be a challenge, usually tackled via ad-hoc definitions. We show that the standard characterisations of the must-preorder carry over as they stand to asynchronous communication, if servers are enhanced to act as forwarders, i.e. they can input any message as long as they store it back into the shared buffer. Our development is constructive, is completely mechanised in Coq, and is independent of any calculus: our results pertain to Selinger output-buffered agents with feedback. This is a class of Labelled Transition Systems that captures programs that communicate via a shared unordered buffer, as in asynchronous CCS or the asynchronous pi-calculus. We show that the standard coinductive characterisation lets us prove in Coq that concrete programs are related by the must-preorder. Finally, our proofs show that Brouwer's bar induction principle is a useful technique to reason on liveness preserving program transformations.

==> coinductive-char.tex <==
%%%%COUNTER EXAMPLE COMPLETENESS HENNESSY CASTELLANI 1998
\section{Co-inductive characterisation of the \mustpreorder}
\label{sec:coinductive-char}


\begin{definition}[Co-inductive characterisation of the \mustpreorder]
\label{def:coinductive-char}
For every finite LTS $\genlts_\StatesA$, $\genlts_\StatesB$ and every
$X \in \pparts{\StatesA}, \serverB \in \StatesB$,
the coinductive characterisation $\coindleq$ of the \mustpreorder is defined as the greatest relation
such that whenever $X \coindleq \stateB$, the following requirements hold:
\begin{enumerate}
\item $X \downarrow \text{ implies } \serverB \downarrow$,
\item\label{pt:coind-tau-serverB} For each $\serverB'$ such that $\serverB \st{\tau} \serverB'$, we have that $X \coindleq \serverB'$,

\item\label{pt:coind-acceptance-sets}
  $X \downarrow$ and $\serverB \stable$ imply that there exist
  $\state \in X$ and $\stateA \in \StatesA$ such that
  $\state \wt{} \stateA \stable$ and $O(\stateA) \subseteq O(\stateB)$,

\item\label{pt:coind-continuations-mu} For any $\mu \in \Act$,
  if $X \cnvalong{\mu}$,
  then for every  $X'$ and $\stateB'$
  such that $X \wt{\mu} X'$ and $\stateB \st{\mu} \stateB'$,
%  $X' \in  \pparts{\StatesA}$ and $\stateB \in \StatesB$
 % such that 
  we have that
  $X' \coindleq \serverB'$.
\end{enumerate}
\end{definition}


\begin{theorem}
\label{thm:coinductive-char-equiv}
For every LTS $\genlts_\StatesA$, $\genlts_\StatesB \in \oba$, every
$\state \in \StatesA$ and $\serverB \in \StatesB$, we have that
$\state \testleqS \serverB$ if and only if $FW(\set{\state}) \coindleq FW(\serverB)$ .
\end{theorem}

\newcommand{\Rfw}{\mathrel{\R_{\textsf{fw}}}}
\newcommand{\Rbase}{\mathrel{\R_{\textsf{base}}}}

\gb{
  We can now prove \req{mailbox-hoisting}. To this end
  recall that $p = \tau.(\co{\aa} \Par \co{b}) \extc \tau.(\co{\aa} \Par \co{c})$
  and $q = \co{\aa} \Par (\tau.\co{b} \extc \tau.\co{c})$.
  First we gather together the pairs due to the transitions on the standard LTS:
  let
  $$
  \begin{array}{lll}
    \Rbase & = &
    \set{ (\set{ p }, q), (\set{ p }, \co{\aa} \Par \co{b}), (\set{ p },  \co{\aa} \Par \co{c}) }
    \\
    & \cup & \set{ (\set{ \co{b}, \co{c} },  \tau.\co{b} \extc \tau.\co{c}) }\\
    & \cup & \set{ (\set{  \co{b}, \co{c} }, \co{b}),   (\set{ \co{b}, \co{c} }, \co{c})}\\
    & \cup & \set{ (\set{ \co{\aa} },  \co{\aa}) }
    \\
    & \cup & \set{ (\set{ \Nil }, \Nil) }
  \end{array}
  $$
  and let
  $$
  \liftFW{ \R } = \setof{ (\liftFW{ X }, \liftFW{ \stateB }) }{ X \R q }
  $$
  The relation $\liftFW{\Rbase}$ does not satisfy the fourth condition on continuations,
  because for instance
  $$
  (\set{ \Nil } \triangleright \varnothing) \wt{ \aa } \set{ \Nil }  \triangleright \mset{ \co{\aa} },
  \qquad
  (\Nil \triangleright \varnothing) \st{ \aa } \Nil  \triangleright \mset{ \co{\aa} }.
  $$
  and $(\set{ \Nil }  \triangleright \mset{ \co{\aa} },  \Nil  \triangleright \mset{ \co{\aa} }) \not \in {\liftFW{\Rbase}}$.
  The first intuition thus is to close binary relations wrt mailboxes via the following function:
  $$
  \begin{array}{lll}
    f_1(\R) & = &\setof{ (X \Par \mailbox{ \Pi M },  q \Par \mailbox{ \Pi M })  }{ X \R q }
%    f_2(\R) & = & \setof{ (X ,  q \Par \mailbox{ \Pi M })  }{ X \R q } \\
  \end{array}
  $$

  Observe that\footnote{If the equivalence via $\doteq$ is not true, then we have use to use strong bisimilarity $\sim$.}
  $$
  \liftFW{ \server \Par \mailbox{ \Pi M } } =
  (\server \Par \mailbox{ \Pi M }) \triangleright \varnothing
  \doteq
  \server \triangleright M
  $$

  We are now ready to unfold the proof.

  \begin{lemma}
    $ \serverA \testleqS \serverB$.
  \end{lemma}
  \begin{proof}
    Let $\hat{\R} = {\liftFW{\Rbase}} \cup f_1(\liftFW{\Rbase})$.
    By construction
    $$
    \liftFW{ \set{ \serverA } } \mathrel{\hat{\R}} \liftFW{ \serverB },
    $$
    and thus \rthm{coinductive-char-equiv} ensures that it suffices to show that
    the relation~$\hat{\R}$ satisfies the conditions in \rdef{coinductive-char}.
    
    Since~$\Rbase$ satisfies \rdefpt{coinductive-char}{coind-tau-serverB},
    WHY DOES $\hat{\R}$ satify the property?

    Since~$\Rbase$ satisfies \rdefpt{coinductive-char}{coind-acceptance-sets},
    \rlem{liftFW-preserves-coind-acceptance-sets} and \rlem{f1-preserves-coind-acceptance-sets}
    imply that~$\hat{\R}$ satisfies \rdefpt{coinductive-char}{coind-acceptance-sets}.

    Since~$\Rbase$ satisfies \rdefpt{coinductive-char}{coind-continuations-mu}
    \rlem{preservation-coind-continuations-mu-1} and \rlem{preservation-coind-continuations-mu-2}
    imply that also~$\hat{\R}$ satisfies that property.
  \end{proof}


  \begin{lemma}
    \label{lem:liftFW-preserves-coind-acceptance-sets}
    Suppose a relation $\R$ satisfies \rdefpt{coinductive-char}{coind-acceptance-sets},
    and for every $(Y,q) \in {\R}$ the processes in $Y$ does not perform input actions.
    Then \rdefpt{coinductive-char}{coind-acceptance-sets} is satisfied also by the relation $\liftFW{\R}$.
  \end{lemma}

  
  \begin{lemma}
    \label{lem:f1-preserves-coind-acceptance-sets}
    Suppose a relation $\R$ satisfies \rdefpt{coinductive-char}{coind-acceptance-sets},
    and for every $(Y,q) \in {\R}$ the processes in $Y$ does not perform input actions.
    Then \rdefpt{coinductive-char}{coind-acceptance-sets} is satisfied also by the relation $f_1(\R)$.
  \end{lemma}
  \begin{proof}
    Fix a pair $(X, q) \in f_1(\R)$ and suppose that $q \stable$ and $X \conv$.
    We have to show that for some $ O \in \acc{X}{\varepsilon}$ such that $O \subseteq O(q)$.
    By construction we know that for some multiset of output actions $M$, set $Y$,
    and process $q'$ we have that 
    $(Y, q') \in {\R}$, $q = q' \Par \mailbox{\Pi M}$ and
    $X = \setof{ (p \Par \mailbox{\Pi M}) }{ p \in Y } $.

    We know by hypothesis that there exists a set $\hat{O} \in \acc{Y}{\varepsilon}$
    such that $\hat{O} \subseteq O(q')$.
    We thus obtain $ \hat{O}\cup M \subseteq O(q') \cup M$,
    and thus $\hat{O} \cup M \subseteq O(q)$.
    Since $\hat{O} \cup M \in \acc{X}{\varepsilon}$ we can conclude.\qed
  \end{proof}


  %% \begin{lemma}
  %%   Suppose a relation $\R$ satisfies \rdefpt{coinductive-char}{coind-acceptance-sets},
  %%   and for every $(Y,q) \in \R$ the processes in $Y$ performs only output actions.
  %%   Then the condition is satisfied also by the relation $f_2(\R)$.
  %% \end{lemma}
  %% \begin{proof}
  %%   Fix a pair $(X, q) \in f_2(\R)$ and suppose that $q \stable$ and $X \conv$.
  %%   We have to show that for some $ O \in \Acc{X}{\varepsilon}$ we have $O \subseteq O(q)$.
  %%   By construction we know that for some multiset of output actions $M$,
  %%   and process $q'$ we have that $(X, q') \in \R$, $q = q' \Par \mailbox{\Pi M}$.

  %%   We know by hypothesis that there exists a set $\hat{O} \in \Acc{X}{\varepsilon}$
  %%   such that $\hat{O} \subseteq O(q')$.
  %%   We thus obtain $ \hat{O} \subseteq O(q') \cup M$,
  %%   and thus $\hat{O} \subseteq O(q)$.
  %%   Since $\hat{O} \in \acc{X}{\varepsilon}$ we can conclude.\qed
  %% \end{proof}


    
  \begin{lemma}
    For any $\R$ that satisfies \rdefpt{coinductive-char}{coind-continuations-mu},
    then also the relation $\liftFW{\R} \cup f_1(\liftFW{\R})$ satisfies \rdefpt{coinductive-char}{coind-continuations-mu}.
  \end{lemma}

  


  
  \begin{lemma}
    \label{lem:preservation-coind-continuations-mu-1}
    For any $(X, \serverB) \in {\Rbase}$,
    and any $\mu \in \Act$,
    such that $\liftFW{X} \cnvalong{\mu}$, $\liftFW{X} \wt{\mu} X'$ and $\liftFW{\stateB} \st{\mu} \stateB'$,
    we have that $(X', \serverB') \in \liftFW{\Rbase } \cup f_1(\liftFW{\Rbase} )$.
  \end{lemma}
  \begin{proof}
    Fix a pair $(X, q) \in {\Rbase}$, %
    a visible action $\mu$ such that $X \cnvalong{\mu}$
    and $\liftFW{ X } \wt{\mu} X'$ and $\liftFW{\stateB} \st{\mu} \stateB'$
    for some $ X'$ and $\serverB'$.
    
    We know by definition of $\liftFW{-}$ that 
    $$
    \begin{array}{lll}
      \liftFW{ X } & = & X \triangleright \varnothing,\\
      \liftFW{ \stateB } & = & \stateB \triangleright \varnothing.
    \end{array}
    $$

    
    We proceed by case analysis on the rule used to derive the transition
    $$
    \liftFW{\stateB} \st{\mu} \stateB'.
    $$
    According to \rfig{rules-liftFW-appendix}
    there are four cases, but \rname{L-Comm} cannot have been used,
    because~$\mu$ is a visible action, and \rname{L-Mout} cannot have been used either,
    because in~$\liftFW{\stateB}$ the mailbox is empty.


    If rule \rname{L-Proc} was used, then the transition is due to the standard LTS,
    so for some $\hat{\stateB}$ we have that
    $$
    \begin{array}{l}
      \stateB' = \hat{\stateB} \triangleright \varnothing,\\
      \stateB \st{\mu} \hat{\stateB}
    \end{array}
    $$
    moreover the construction of $\Rbase$ ensures that $\mu$ is an output action.
    
    We now reason on the weak transition $ \liftFW{ X } \wt{ \mu } X'$.
    Wi discuss first the special case in which the transition is actually strong, i.e. there are no tau steps.
    The transition at hand must be due to either \rname{L-Proc} or \rname{L-Mout}, but
    in $ \liftFW{ X } $ the mailbox is empty, hence the transition cannot
    be due to \rname{L-Mout}. This means that the transition is due to the standard LTS, so for
    some $\hat{X}$ we have
    $$
    \begin{array}{l}
      X' = \hat{X} \triangleright \varnothing,\\
      \hat{ X } \st{\mu} \hat{X}.
    \end{array}
    $$
    But then $( \hat{X}, \hat{\stateB}) \in \Rbase$, because by hypothesis $\R$ satisfies
    \rdefpt{coinductive-char}{coind-continuations-mu}.
    It follows that $(X', q') \in \liftFW{\Rbase}$ 

    TODO: discuss the case in which there are taus before or after the action $\mu$.

    
    If the rule \rname{L-Minp} was used, then
    $$
    \stateB' = q \triangleright \mset{\co{\mu}},
    $$
    the action $\mu$ is an input.
    The construction of $\Rbase$ ensures that $X$ performs only output actions,
    hence the transition $\liftFW{ X } \st{\mu} X' $ must be due to
    the rule  \rname{L-Minp}, and thus
    $$
    X' = X \triangleright \mset{\co{\mu}}
    $$
    It follows that $(X', q') \in f_1(\liftFW{\Rbase})$.

    TODO: discuss the case in which there are taus before or after the action $\mu$. \qed
  \end{proof}

  

  
  \begin{lemma}
    \label{lem:preservation-coind-continuations-mu-2}
    For any $(X, \serverB) \in f_1( \Rbase )$,
    and any $\mu \in \Act$,
    such that $\liftFW{X \cnvalong{\mu}}$, $\liftFW{X} \wt{\mu} X'$ and $\liftFW{\stateB} \st{\mu} \stateB'$,
    we have that $(X', \serverB') \in \liftFW{\Rbase} \cup f_1(\liftFW{\Rbase} )$.
  \end{lemma}
  \begin{proof}
    Fix a pair $(X, q) \in f_1(\Rbase)$ and a visible action $\mu$ such that $X \cnvalong{\mu}$
    and $\liftFW{ X } \wt{\mu } X' $ and $\liftFW{\stateB} \st{\mu} \stateB' $.

    By construction for some $M$ we have
    $$
    \begin{array}{lll}
      \liftFW{ X } & = & (X \Par \mailbox{\Pi M}) \triangleright \varnothing,\\
      \liftFW{ \stateB } & = & (\stateB \Par \mailbox{\Pi M}) \triangleright \varnothing.
    \end{array}
    $$

    We proceed by case analysis on the rule used to derive the transition
    $\liftFW{\stateB} \st{\mu} \stateB' $.
    According to \rfig{rules-liftFW-appendix}
    there are four cases, but \rname{L-Comm} cannot have been used,
    because~$\mu$ is a visible action, and \rname{L-Mout} cannot have been used either,
    because in~$\liftFW{\stateB}$ the mailbox is empty.

    Case \rname{L-Proc}
    
    TODO: FINISH ME

    Case \rname{L-Minp}

    TODO: FINISH ME

    
    \bigskip
    
    OLD PROOF. AVOID IT.
    
    Either the transition of $X$ is due to forwarding or to the standard LTS.
    If the transition is due to forwarding then $X' = \hat{X} \Par \mailbox{\Pi M \Par \co{ \mu} } $
    and $\mu$ is an input action. Since in the original LTS no state can perform any input,
    the transition $\liftFW{\stateB}  \st{\mu} \liftFW{\stateB'} $ must also be due to forwarding,
    thus $q' =  \hat{q} \Par \mailbox{\Pi M \Par \co{ \mu}}$,
    and thus $(X', q') \in f_1(\Rfw)$.

    
    If the transition of $X$ is due to the standard LTS then
    $$
    \hat{X} \Par \mailbox{\Pi M} \wt{\mu} \hat{X}' \Par \mailbox{\Pi M'}
    $$
    and $\mu$ is an output action.
    Either $\hat{X} = \hat{X}'$ or $\mailbox{\Pi M} = \mailbox{\Pi M'}$.

    In the first case  $M' = M \setminus \mset{ \mu }$, and
    $(\hat{X}, \hat{q}) \in \Rfw$.
    We have to find some mailbox $\hat{M}$ such that
    $$
    \begin{array}{lll}
      X' & = & \hat{X}' \cup \Par \mailbox{\Pi \hat{M}}\\
      q' & = & \hat{q}' \cup \Par \mailbox{\Pi \hat{M}}\\
    \end{array}
    $$
    with $( \hat{X}',  \hat{q}') \in \Rfw$.

    If the transition in $q$ is due to the mailbox then
    $q' = \hat{q}$ and thus we have $(\hat{X}' \Par \mailbox{\Pi M'}, \hat{q} \Par \mailbox{\Pi M'}) \in f_1(\Rfw)$.
    If the transition is due to $\hat{q}$ then
    $ q' = \hat{q}' \Par \mailbox{\Pi M}$, and
    output-determinacy implies
    that
    $$
    q' =  \hat{q}' \Par \mailbox{\Pi M} \simeq \hat{q} \Par \mailbox{\Pi M \setminus \mset{ \mu }} = \hat{q} \Par \mailbox{\Pi M'}
    $$
    It now follows that $ (X', q') \in f_1(\Rfw) $.\footnote{Technically, we need to close the relations wrt $\simeq$.}
    \qed
  \end{proof}
  
  }

